Transaction Cost Analytics for Corporate Bonds

The electronic platform has been increasingly popular for executing large corporate bond orders by asset managers, who in turn have to assess the quality of their executions via Transaction Cost Analysis (TCA). One of the challenges in TCA is to build a realistic benchmark for the expected transaction cost and to characterize the price impact of each individual trade with given bond characteristics and market conditions. Taking the viewpoint of retail investors, this paper presents an analytical methodology for TCA of corporate bond trading. Our analysis is based on the TRACE Enhanced dataset; and starts with estimating the initiator of a bond transaction, followed by estimating the bid-ask spread and the mid-price dynamics. With these estimations, the first part of our study is to identify key features for corporate bonds and to compute the expected average trading cost. This part is on the time scale of weekly transactions, and is by applying and comparing several regularized regression models. The second part of our study is using the estimated mid-price dynamics to investigate the amplitude of its price impact and the decay pattern of individual bond transaction. This part is on the time scale of each transaction of liquid corporate bonds, and is by applying a transient impact model to estimate the price impact kernel using a non-parametric method. Our benchmark model allows for identifying abnormal transactions and for enhancing counter-party selections. A key discovery of our study is the price impact asymmetry between customer-buy orders and consumer-sell orders.

==> bond_2020/sections/Section3_dataset_b.tex <==


\section{The dataset: TRACE,  {Thomson Reuters}, Mergent Fixed Income Securities and data processing}\label{data_pre}


Although TRACE Enhanced has more accurate  information on historical traded volume, it may not provide customers timely information to evaluate dealers offers on their intended tradings due to the lag of 6 months. Therefore, we compare the outcome of OLS and two-step LASSO with both TRACE Enhanced  and  TRACE Standard datasets.




As mentioned earlier,  the main obstacle for econometric studies on corporate bonds is the lack of transparency. In all available databases,
some basic yet critical information, such as 
the best executed price for bond tradings, is unavailable. 
Nevertheless, some information, though limited, are recorded in the TRACE database, and have been used for empirical studies by \cite{DICK2014} and \cite{citeulike:13771761}. 
TRACE, an acronym for {\it the Trade Reporting and Compliance Engine}, is the FINRA-developed mechanism that facilitates the mandatory reporting of OTC secondary market transactions in eligible fixed income securities.

{\color{red}
FINRA provides two types of TRACE datasets, TRACE Standard dataset and TRACE Enhanced dataset, along with a separate dataset for monthly price, return, coupon and yield information for all corporate bonds traded since July 2002. Both TRACE Standard dataset and TRACE Enhanced dataset contain corporate bond transactions. The difference is that transactions are available on TRACE Standard with a two weeks of delay but the volume of the transaction is capped at 1MM for high yield bonds and 5MM for  investment grade bonds. TRACE Enhanced dataset has the uncapped volume but transactions are available with a delay of 6 months. Although TRACE Enhanced dataset has more accurate  information on historical traded volume, it may not provide customers with timely information to evaluate dealers' offers on their intended tradings due to the time lag.  To avoid truncation issues, we focus on TRACE Enhanced dataset to understand the price formation of bonds. Moreover, we also compare the results for some regression methods with both TRACE Enhanced dataset  and  TRACE Standard dataset. See Section \ref{sec:two_trace_comparison}.



%The main difficulty to work with TRACE comes from the lack of information on the liquidity offer. For example, there are neither quotes,  nor bids price, nor asks price. In TRACE, only transactions are recorded, together with the type of the transaction: dealer-to-dealer, dealer-to-customer, or customer-to-customer. %But  volumes of the trade in TRACE are truncated: % if the transaction volume is above one million dollars  for individual investor (or  five million dollar for institutional trades), only the minimum between the real size of the transaction and one million (or five million for institutional trades) is recorded.

The main difficulty to work with TRACE comes from the lack of information on the liquidity offer. For example, there are neither quotes,  nor bids price, nor asks price. In TRACE, only transactions are recorded, together with the type of the transaction: dealer-to-dealer, dealer-to-customer, or customer-to-customer.  To address this issue,
 we will use the untruncated transaction volumes on Enhanced TRACE along with other information to construct the estimation of bid-ask spread (Section \ref{preliminary}).} The data  we use is  from January 1st 2015 to December 31st 2016, and obtained from Wharton WRDS. In this period, there are 34,809,405 original trade reports, 390,193 reports of trade cancellations (approximately 1.1 percent of all original trade reports), 497,249 corrected trade reports (about 1.4 percent), and 28,005 reports of trade reversals. Trade reversals are transactions that have been changed after more than 20 days since they were initially recorded. Occasionally there are  multiple correction records for the same original trade
 and cancel records that  cancel  previously corrected trades. We will address the data cleaning procedure below. There are 54,885 CUSIP\footnote{CUSIP stands for {\it Committee on Uniform Securities Identification Procedures}.}-days spread over 656 calendar days, many of which are weekends and holidays. The CUSIP-days are computed by {counting} all the trade days over all the CUSIP bonds.
 
 
 
 In particular, for each transaction  of a bond, one can recover from Enhanced TRACE the following information:
 \begin{itemize}
\item $t^b_k$: the timestamp for the $k$th transaction of bond $b$;
\item $P^b_k$: the price of  the $k$th transaction of bond $b$;
\item $V^b_k$ : the volume of the $k$th transaction of bond $b$;
\item the side of the dealer-to-customer transaction: customer buy order or customer sell order.
\end{itemize}
  {
 We rely on Thomson Reuters to retrieve information  on the bonds traded, such as the amount issued, the coupon rate, the sector information, and rating information. {\color{red}The outstanding amount is accessed in Mergent Fixed Income Securities Database (FISD).} Thomson Reuters also provides data on the Libor and Overnight Indexed Swap rate.}
 
 
 
\subsection{Data filtering}\label{filtering}
The data cleaning procedure combines the approaches in \cite{DICK2014} and \cite{citeulike:13771761}, with  the following steps: 
\begin{enumerate}
\item Remove canceled trades and apply corrections to ensure that only trades that are actually settled are accounted for. After the removal of canceled trades and  canceled corrections records, there are 32,931,539 trades.

\item Since both principal and agent in the dealer-to-dealer transactions will report their transaction to FINRA  (see \cite{DICK2014}),
 remove the ones reported by agents. As a result,  2,095,934 (i.e. 6.36\%) of the reports are removed, with 30,835,605 reports remaining after this step.

\item Remove the transactions in unusual trading days  such as weekends and holidays. Thus 
5,753 (0.02\%) records are removed, with  30,829,852 reports left after this step.

\item Exclude all trade reports with execution time outside of the normal 8:00AM to 5:15PM ET trading hours. Therefore, 745,619 (i.e. 2.4\%) are removed, with  30,084,233 reports remaining after this step. 

\item Remove all irregular trades with sales condition codes that indicate late reports, late reports after market hours, weighted average price trades, or trades with special price flags. As a result, 583,157 (i.e. 1.9\%) reports are removed, with  29,501,076 reports left after this step. 


\item Remove trade reports with price below 10 (percentage points of 100). This price filter step excludes 217,321 (i.e. 0.74\%) of the remaining trades, with 29,283,755 reports left after this step.

\item Select reports classified as {\it corporate bonds} in the dataset. Remove those reports with sub-product indicators such as Mortgage Backed Securities Transactions. Consequently, 563,942  (i.e. 1.94\%) of the remaining reports are filtered out, with 28,719,813 reports  left.
\end{enumerate}
In total, about 17.50\% reports are filtered out from the original Enhanced TRACE dataset. Among all the remaining 28,719,813 records, 14,071,375 (i.e. 49\%)  are Dealer-to-customer trades and the remaining 14,648,438 (i.e. 51\%) are trades between dealers. 
These statistics are summarized in Table \ref{tbl:data_clean}.


\begin{table}[ht]\small{
    \centering\captionsetup{margin = 1.5cm}
    \caption{Data filtering procedure.}
    \label{tbl:data_clean} 
    \setlength{\tabcolsep}{8pt}
    \captionsetup{margin=2.5cm}
    % \hspace*{-5ex}\begin{tabular}{@{}l
    %                 *{7}{S[table-format=5.2,table-number-alignment=center]}@{}}
    %                 \toprule
    %                 { }& {Step 1} & {Step 2} & {Step 3} & {Step 4} & {Step 5} & {Step 6} & {Step 7} \\
    %                 { }& {Settled}& {Dealer}& {Usual days}& {Usual hours}& {Regular}& {Price}& {Bonds}\\ \midrule
    %                 Removal (total)&1,877,866&2,095,934&5,735&745,619&583,157&217,321&563,942\\
    %                 Removal (percentage) &{5.4\%} & {6.36\%}&{0.02\%}&{2.4\%}&{1.9\%}&{0.074\%}&{1.94\%}\\
    %                 Number left&32,931,539&30,835,605&30,829,853& 30,084,233&29,501,076&29,182,755&28,719,813\\ \bottomrule
    %               \end{tabular}
    \begin{center}
      \begin{tabular}{lrrr}
        &Removal (nbe)& Removal (pct)& Number left\\\toprule
        Step 1\\
        Keep settled trades &1,877,866 &{5.4\%} &32,931,539\\\midrule
        Step 2\\
        Keep trades reported by dealers &2,095,934 & {6.36\%}&30,835,605\\\midrule
        Step 3\\
        Keep business days  &5,735 &{0.02\%}&30,829,853\\\midrule
        Step 4\\
        Keep opened hours  &745,619 &{2.4\%}& 30,084,233\\\midrule
        Step 5\\
         Keep regular trades           &583,157 &{1.9\%}&29,501,076\\\midrule
        Step 6\\
        Keep compatible prices                              &217,321 &{0.074\%}&29,182,755\\\midrule
        Step 7\\
        Keep bonds only                    &563,942 &{1.94\%}&28,719,813\\\midrule
        Selection LR\\
        For bid-ask spread regression & -- & -- & 4,371,363\\\midrule
        Selection PI\\
        For price impact curves & -- &-- & 3,564,264\\
        \bottomrule
      \end{tabular}
    \end{center}
            }
\end{table}

\subsection{Bond selection for linear regression}\label{bond_selection_regression}
The regression analysis  includes two types of bonds:  investment grade bonds and high yield bonds. The investment grade bonds are selected from iShares iBoxx \$ Investment Grade Corporate Bond ETF and the high yield bonds are selected from the components of iShares iBoxx \$ High Yield Corporate Bond ETF.
There are 1,033 current holdings of the former, among which {\color{red}538} bonds have more than one transaction recorded in Enhanced TRACE during the time period of Jan 1st, 2015 to Dec 31, 2016. These {\color{red}538} bonds are selected in the regression analysis.
There are 1,575 current holdings of the latter, 1485 of which have transaction records during the same period. Moreover, there are 
30 bonds that belong to both iShares iBoxx \$ High Yield Corporate Bond ETF and iShares iBoxx \$ Investment Grade Corporate Bond ETF.
 The rating levels of all these 30 bonds  have been adjusted since issuance. Hence there are total of  1,993 bonds in the regression analysis.


 After data cleaning, there are 14,071,375 trading reports between dealers and customers. Even though only  1,993 bonds are selected, these selected bonds consist of 31.05 \% of the total filtered customer-to-dealer reports. %\cmt{could this be considered as a filter?}
Table \ref{tbl:data_clean}  reports this selection as ``Selection LR'', and Table~\ref{tbl:statistics_1993} reports the statistics of these selected bonds. See also Table~\ref{tbl:RPT-1993} and Table~\ref{tbl:nonRPT-1993} for the statistics of RPTs and non-RPTs.

 {RPT stands for the {\it Riskless principle trade}. Detailed discussion on RPT is
in Section \ref{sec:RPT}.} Our percentage of RPTs is lower than that reported in \cite{citeulike:13771761}, partly  because of different dataset with a different time period. \cite{citeulike:13771761} used TRACE data from April 1, 2014 to March 31, 2015. In addition, in the TRACE data, the markers (``1MM+" and ``5MM+") for larger trades assign the same value to many large trades.  Finally, we only count the RPTs for a subset of bonds whereas \cite{citeulike:13771761} estimated the PRTs for a larger set of bonds.  


\begin{table}[H]
\centering\captionsetup{margin = 2.5cm}
\small{
\begin{center}
\setlength{\tabcolsep}{4pt}
\captionsetup{margin=2.5cm}
\hspace*{-4ex}\begin{tabular}{@{}l
*{4}{S[table-format=10.2,table-number-alignment=center]}@{}}
\toprule
{}&{Total}&{Investment Grade}&{High Yield}&{Bonds with rating changes}\\\midrule
    Number of trades& 4,371,363&3,102,791&1,109,177&159,395\\
    Number of Customer buy &2,549,932&1,834,873&623,839&91220\\
    Number of Customer sell &1,821,371&1,267,888&485,308&68175\\ 
    Total trading volume  (billion)&3,401.76 &2,438.26 &850.46&113.04\\
   % (billion)&&&&\\
     Avg trading volume &778,202.926&785,834.74&766,775.08&709,163.43\\
     % (sd)   &{(22.70)}&{(25.40)}&{(14.03)}&{(13.92)}\\
     Avg price &102.05&104.26&97.81&88.58\\
   %  (sd) &{(0.00006)}&{(0.00005)}&{(0.00007)}&{(0.00007)}\\
    Prop Volume of Customer buy &55.3\%&56.8\%&51.7\%&58.2\%\\
    Prop Volume of Customer sell &44.7\%&43.2\%&48.3\%&41.8\%\\ \bottomrule
\end{tabular}
\caption{Description of selected 1,993 bonds for regression (dealer-customer trades).}
\label{tbl:statistics_1993} 
\end{center}}
\end{table}




%\begin{table}[H]
%\centering\captionsetup{margin = 2.5cm}
%\small{
%\begin{center}
%\caption{Description of selected 1993 bonds for regression (dealer-customer trades).}
%\label{tbl:statistics_1993} 
%\setlength{\tabcolsep}{8pt}
%\captionsetup{margin=2.5cm}
%\begin{tabular}{@{}l
%*{4}{S[table-format=10.2,table-number-alignment=center]}@{}}
%\toprule
%{}&{Total}&{Investment Grade}&{High Yield}&{Bonds with rating changes}\\\midrule
%    Number of trades& 4,371,363&3,102,791&1,109,177&159,395\\
%    Number of Customer buy &2,549,932&1,834,873&623,839&91220\\
%    Number of Customer sell &1,821,371&1,267,888&485,308&68175\\ 
%    Total trading volume &3,401,760,788,827.9&2,438,257,395,349.7&850,466,287,144.2&113,037,106,334.0\\
%     Avg trading volume &778,202.926&785,834.74&766,775.08&709,163.43\\
%         &{(22.70)}&{(25.40)}&{(14.03)}&{(13.92)}\\
%     Avg price &102.05&104.26&97.81&88.58\\
%      &{(0.00006)}&{(0.00005)}&{(0.00007)}&{(0.00007)}\\
%    Prop Volume of Customer buy &55.3\%&56.8\%&51.7\%&58.2\%\\
%    Prop Volume of Customer sell &44.7\%&43.2\%&48.3\%&41.8\%\\ \bottomrule
%\end{tabular}
%\end{center}}
%\end{table}



\subsection{Bond selection for price impact analysis}\label{sec:price_imapct_bond_statistics}
%\cmt{could this be considered as another filter? tables could go in appendix, I am not sure RPT stats are really important for them}
Among all the 1,993 bonds for regression analysis, the top-{\color{red}200} traded bonds, {\color{red}in terms of number of transactions,} are selected to calculate the price impact curves since the calculation requires higher trading frequency. Table \ref{tbl:data_clean} report this selection as ``Selection PI'', and Table~\ref{tbl:statistics_1000} summarizes statistics of these {\color{red}200} bonds. {\color{red}Comparing Tables \ref{tbl:statistics_1993} and \ref{tbl:statistics_1000}, we see that top-200 bonds account for 32\% of the total number of transactions among 1993 bonds.} Note that among the $30$ bonds with rating level adjustment, {\color{red}$13$} of them belong to the top-{\color{red}200} traded bonds. Table~\ref{tbl:RPT} and Table~\ref{tbl:nonRPT} report the potential RPTs and non-RPT dealer-customer trades of the top-{\color{red}200} traded bonds. 



\begin{table}[H]
\centering\captionsetup{margin = 2.5cm}
\small{
\begin{center}
\setlength{\tabcolsep}{5pt}
\captionsetup{margin=2.5cm}
\hspace*{-4ex}\begin{tabular}{@{}l
*{4}{S[table-format=10.2,table-number-alignment=center]}@{}}
\toprule
{}&{Total}&{Investment Grade}&{High Yield}&{Bonds with rating changes}\\\midrule
    Number of trades&1,404,507& 980,005 &309,777&116,561\\
    Number of Customer buy &836,825&588,128&180,378&68,319\\
    Number of Customer sell &567,682&390,537&128,903&48,242	\\ 
    Total trading volume (billion)&605.5 &430.83 &107.70&66.98\\
   % (billion)&&&&\\
     Avg trading volume &431,119.48&440,217.83&348,241.14&574,636.26\\
     Avg price &100.08&103.32&94.58&87.55\\
     Prop Volume of Customer buy &52.2\%&53.12\%&50.1\%&49.6\%\\
    Prop Volume of Customer sell &47.8\%&46.88\%&49.9\%&50.4\%\\ \bottomrule
\end{tabular}
\caption{Description of selected {\color{red}200} bonds for {\color{red}price impact analysis} (dealer-customer trades).}
\label{tbl:statistics_1000} 
\end{center}}
\end{table}




\subsection{Preliminary data analysis}\label{preliminary}
To analyze price impact, there are several important quantities to estimate, the first one being to identify the initiator of a transaction.

\paragraph{Identifying the initiator of a transaction and RPTs.}\label{sec:RPT}
For equity shares,  the initiator of a trade, say in a limit order book, is clearly the liquidity consumer. This is not the case for bond trading where  a trade is characterized by both the type of transaction (buy or sell) {\it and} who has initiated the trade.

\cite{citeulike:13771761} identified a significant fraction of  transactions between dealers and customer as RPT (\emph{riskless principal trade}). {This corresponds to the situation where the dealer has found two clients, and put herself in between the transactions.} As a consequence, it is not possible to recover the initiator of the RPT as it is difficult to determine  which of the two clients called first and hence who initiated the trades. 

To identify the initiator of a bond trade, we rely on the Enhanced TRACE data  to identify each trade as either a buy or a sell type,  assuming the client is always the liquidity consumer, and the dealer is always the liquidity provider. We target to further assign to each trade a sign of +1 when it has been initiated by a buyer, and -1 when it has been initiated by a seller. 
Our methodology is described in Appendix \ref{sec:signtrades}.

After identifying all the potential  RPTs, we consider the transaction initiated by the client. We define the \emph{sign of the transaction $\epsilon^b_k$} as $+1$ (i.e., ``buy'') if a client buys from a dealer, and $\epsilon^b_k$ as
$-1$ (i.e., ``sell'') if a client sells to a dealer. When it is not possible to determine the sign of a trade as in the above RPT case, we will assign $\epsilon_k^b$ to be zero. 

\paragraph{Bid-ask spread estimation.}
After identifying the trade, it is possible to estimate the bid-ask spread $\psi^b_k$, and hence the \emph{mid-price} $M^b_k$ for each transaction $k$ of bond $b$, using the following methodology.


First find two consecutive trades which have opposite signs $\epsilon_{k+1}=-\epsilon_{k}$ with $\epsilon_{k}\ne 0$,
and which are sufficiently close in time (i.e., $|t^b_{k+1}-t^b_k|<\Delta t$), and define the estimate of the vanilla bid-ask spread as
\begin{eqnarray} \label{estimated_vanilla_spread}
\psi^b_{k+1}:=(P^b_{k+1}-P^b_k)\cdot \epsilon^b_{k+1}.
\end{eqnarray}
The mid-price at $t_k$ is then estimated by 
\begin{equation}
M^b_k:=P^b_k - \epsilon^b_{k+1} \,\frac{\psi^b_{k+1}}{2}.
\end{equation}
{\color{red}Then we can formally introduce the bid-ask spread (in basis point) adopted in this paper
\begin{eqnarray} \label{estimated_spread}
s^b_{k+1}:=\frac{\psi^b_{k+1}}{M^b_k} \times 10000.
\end{eqnarray}}
In this paper, we choose  $\Delta t=5$-minute because of the low
trading frequency of the corporate bond market.\footnote{\color{red}$\Delta t<1$-minute is too small for illiquid market like corporate bond. On the other hand, having $\Delta t\ge 10$-minute leads to the lack of sufficient data. We have checked the results with $\Delta t=4$-minute and $\Delta t=6$-minute which provide similar results compared to $\Delta t=5$-minute, indicating a stable choice of $\Delta t=5$-minute.} {As a consequence, only 15.6\% of the transactions are used to calculate the bid-ask spread among bonds that are selected from Section \ref{bond_selection_regression}.} 

To check the reliability of these estimates as only 15.6\% of the trades are used to compute them, we compare the estimated bid-ask spread with the one computed using bid and ask quotes provided by Composite Bloomberg Bond Trader (CBBT) for those bonds that are available in both CBBT and Enhanced TRACE data set. CBBT  is a composite price based on the most relevant executable quotations on FIT, Bloomberg's Fixed Income Trading platform. 
CBBT pricing source provides average bid-ask prices based on executable quotes that are listed on Bloomberg's trading platform. Its aim is to indicate where clients can reasonably expect to execute on the platform during trading hours, and prices are updated as dealer levels change. \cite{FGP2016} used the CBBT data as a measure of bond liquidity. {We only have access to} quote price data from Bloomberg CBBT %is available
from June 1st, 2015 to  May 31, 2016 (12 months) for 2,361 investment grade bonds that belong to the iboxxIG universe. The iboxxIG universe is the standard universe for U.S. investment grade corporate bond. Among these 2,361 bonds, we {identified} %choose
1,401 bonds which have records in both Bloomberg CBBT database and Enhanced TRACE subset.

Figure \ref{fig:spread_empirical} below shows the  plot for the empirical distribution of the spread from CBBT and the estimated spread from Enhanced TRACE for two arbitrarily chosen bonds, whose statistics are reported  in Table \ref{tbl:spread}.
It is noticeable (and expected)  that the CBBT spreads are larger than the estimated ones from real trades available in Enhanced TRACE. \cite{FGP2016} pointed out, CBBT bid-ask spread estimates are based on quotes, and not on real transactions, as a consequence they include quotes that are not attractive enough (i.e. not small enough) to trigger a transaction. Since the bid-ask spread is the first component of implicit transaction costs, trades occur when they are smaller than the average bid-ask spread.
%Because of its focus on transaction costs, our paper focuses on 


%{\bf \color{green} DONE: why CBBT has bigger spread? reference from Charles}. 

\begin{figure}[ht]
\centering
        \begin{subfigure}[b]{0.5\textwidth}
                \centering
                \includegraphics[width=\textwidth]{figs/spread_comparison_US375558BG78.pdf}
                \caption{US375558BG78}
                \label{fig:gull}
        \end{subfigure}%
        \begin{subfigure}[b]{0.5\textwidth}
                \centering
                \includegraphics[width=\textwidth]{figs/spread_comparison_US126650CJ78.pdf}
               \caption{US126650CJ78}
                \label{fig:gull2}
        \end{subfigure}%
\caption{Empirical distributions of the spread {\color{red}(Eqn \eqref{estimated_spread}}).}\label{fig:spread_empirical}
\end{figure}

%

\begin{table}[ht]
\centering\captionsetup{margin = 2.5cm} 
\setlength{\tabcolsep}{8pt}
\captionsetup{margin=2.5cm}
\begin{tabular}{@{}l
*{6}{S[table-format=2.1,table-number-alignment=center]}@{}}
\toprule
{ } &{Coupon} & {Amount outstanding} & \multicolumn{2}{c}{Average spread (bp)} &
\multicolumn{2}{c}{Daily average} \\
  { } &{} & {} & \multicolumn{2}{c}{} &
\multicolumn{2}{c}{number of updates} \\ 
 \cmidrule(lr){4-5}\cmidrule(lr){6-7}         
{ } &{ }& {(USD)} & {CBBT} & {TRACE} &
{CBBT} & {TRACE}  \\ \midrule
US375558BG78 &4.6\% &\,\, 1,000,000,000 &118.78&66.24&2336.49&1.63\\
    US126650CJ78 &2.8\% &\,\,\,\,2,750,000,000&45.12&29.88&3406.20&11.50\\ \bottomrule
\end{tabular}
\caption{Spread comparison.}
\label{tbl:spread}
\end{table}

\begin{table}[H]
\centering\captionsetup{margin = 2.5cm} 
\setlength{\tabcolsep}{4pt}
\captionsetup{margin=2.5cm}
\begin{tabular}{@{}l
*{7}{S[table-format=6.2,table-number-alignment=center]}@{}}
\toprule
{Month }& {1 } & {2} & {3} & {4 } & {5 }&{6} \\ \midrule
Number of observations&1027&823&820&847&890&892\\
25\% & 0.7165&0.655&0.647&0.666&0.655&0.643\\
Median & 0.971 &0.931 & 0.899 & 0.900 & 0.852 &0.873\\
75\% & 1.238 & 1.213 & 1.224 & 1.182 &1.144 & 1.19\\
Mean & 0.970 & 0.956& 0.951& 0.941 &0.920& 0.931\\  \bottomrule
{Month}& {6} & {7} & {8} & {9}  &{10}&{12}\\ \midrule
Number of observations&939&914&1069&1062&1040&1047\\
25\% & 0.705&0.717&0.670&0.643&0.598&0618\\
Median & 0.963&1.000&0.893&0.830&0.779&0.834\\
75\%& 1.289 & 1.309 & 1.182 & 1.090 & 1.056 & 1.130\\
Mean & 0.994 &1.019 &0.941 &0.889 &0.854 &0.893\\ \bottomrule
\end{tabular}
\caption{Statistics of the ratios.}
\label{tab:ratio}
\end{table}

\paragraph{Bid-ask spread stationarity.} We next check the consistency of the two approaches via a stationarity test on the ratio of the two estimates: the CBBT bid-ask spread and our trades-based estimates.
That is, we split the year 2016 by two consecutive months and check if this ratio is stationary from one period of two months to the other. 

Denote $s^{\text{CBBT}}_{b,w}$ as the average spread for bond $b$ over the period $w$ taken from Bloomberg CBBT, and $s^{\text{TRACE}}_{b,w}$ as the {average of the } estimated bid-ask spread for bond $b$ in period $w$ from Enhanced TRACE {\color{red}(Eqn \eqref{estimated_spread})}.
{First of all, note that the empirical estimate of the bid-ask spread using Enhanced TRACE transactions are smaller than the CBBT ones, the average ratio is between 0.9 and 1 and its median is between 0.7 and 1.}
 The statistics of the ratios are summarized in Table \ref{tab:ratio}.
 
%The relative ratio of the spread from Bloomberg and the spread estimated using transaction data from TRACE is defined as $R^{b,w} = \frac{ S^{bloomberg}_{b,w}}{ S^{TRACE}_{b,w}}$. Notice that some bonds are issued after 5/31/2016, hence the data size slightly varies from month to month. Denote  $F_w$ as the empirical distribution of $\{R^{b,w} , \forall b\}$. 
We use two tests for the stationarity of the statistic $R_{b,w}=s^{\text{CBBT}}_{b,w}/s^{\text{TRACE}}_{b,w}$ from one period $w$ to the other $w+1$.
The first is one-way ANOVA test, and the second is Kruskal-Wallis H-test.
{The former tests the stationarity of the mean and the latter tests the stationarity of the median.} The mathematical formulations and definitions of ANOVA test and  Kruskal-Wallis H-test are in Appendix \ref{a_h_tests}.
%The hypothesis in One-way ANOVA test is that population $\{R^{b,w} , \forall b\}$ mean are equal for two consecutive time periods.
% Similarly, the hypothesis in Kruskal-Wallis H-test is that population $\{R^{b,w} , \forall b\}$ medians are equal for two consecutive time periods. Note that rejecting the null hypothesis does not give indication as to which groups differ. Post-hoc comparisons between groups are required to determine which groups are different. 



%\noindent \textbf{Result: } H-statistic=$580.98$, P-value=$1.6e-117$.




\begin{table}[H]
\centering\captionsetup{margin = 2.5cm} 
\setlength{\tabcolsep}{4pt}
\captionsetup{margin=2.5cm}
\begin{tabular}{@{}l
*{7}{S[table-format=6.2,table-number-alignment=center]}@{}}
\toprule
{Month }& { 1 and 2} & {2 and 3} & {3 and 4} & {4 and 5} & {5 and 6} & {6 and 7}\\ \midrule
ANOVA&4.59&0.10&0.39&1.71&0.52&15.32\\
(P-value)&0.032&0.751&0.533&0.191&0.472&0.000\\
H-test&3.564&0.163&0.154&1.890&0.296&15.16\\ 
(P-value)&0.038&0.686&0.6947&0.169&0.586&0.000\\ \bottomrule
{Month  }& {7 and 8} & {8 and 9} & {9 and 10}  &{10 and 11}&{11 and 12}\\ \midrule
ANOVA&2.21&25.54&14.15&6.72&7.81\\
(P-value)&0.136&0.000&0.0001&0.01&0.005\\
H-test    &2.30   &23.78   &12.03  &8.54&5.82\\ 
(P-value) &0.129  &0.000  &0.0005  &0.003&0.015\\ \bottomrule
\end{tabular}
\caption{Results of ANOVA and Kruskal-Wallis H-tests.}
\label{tab:compba}
\end{table}

Table \ref{tab:compba} summarizes the result of both ANOVA test and Kruskal-Wallis H-test. For most of the tests,
with $99\%$ confidence level, we accept the null hypothesis in both ANOVA test and Kruskal-Wallis tests for $7$ out of the total $11$ comparisons. This implies a good stationary property of the ratios over time. 

{We will thus use our estimation of the bid-ask spread in all the following, because it can be operated over years of data using Enhanced TRACE, where CBBT is costly to obtain and linked to a private procedure owned by Bloomberg. Nevertheless, these stationarity tests imply that a large investor using CBBT estimates could rely on the methodology presented thereafter and apply a ratio to read our results in terms of ``units'' of CBBT.}




==> bond_2020/sections/Section4_regression_b.tex <==

\section{Expected Bid-Ask Spread Estimation via Regularized Regressions}
\label{sec:linreg}\label{sec:reglin}
\label{sec:linereg}


%\subsection{Data Analysis via regularized regressions}
 
% -----


In this section, regularized regression models including OLS,  the two-step Lasso, the Ridge,  and the EN regressions, along with a $K$-fold cross-validation method, will be exploited  to pick the optimal parameters for these models. The regression analysis will focus on the trades between customers and dealers, which are  statistically different from  trades between dealers. The analysis for the latter 
 requires more information that are currently missing in the database, including indications of  who initiates the dealer-to-dealer trade.
The regression analysis is performed on a weekly frequency. For each week, the average estimated spread $\psi$ is computed by method in Eqn. \eqref{estimated_spread} for every bond as the response variable. {\color{red}Recall that in Section \ref{bond_selection_regression},  $1,993$ bonds have been selected for the regression analysis. Correspondingly, there are total $152,408$ data samples processed from the TRACE Enhanced dataset during January $2015$ and December $2016$. }

\paragraph{Features and response variables.}
The features in the regression consist of  two categories. One category concerns bond information, including time to maturity date, time since issued date, coupon rate, amount outstanding, and duration. The other category focuses on trade information, including average transaction price, volatility, proportion of costumer-buys (sells), LIBOR-OIS rate, and 5-year treasury rate during the given week. More specifically,
\begin{itemize}
\item {\bf {Bid-ask} spread}:   estimated for each time $t$ using Equation \eqref{estimated_spread}, from which  the weekly average spread is computed  for each bond $b$ in week $w$.
\item {\bf Volatility}: calculated from the trade price. For bond $b$, assume there are $n$ trades in week $w$. Recall $P^b_j$ as the trade price of the $j^{th}$ transaction ($j=0,1,2,\cdots,n$) of bond $b$. Denote the log return $r_{i}^b = ln( \frac{P^b_{i}}{P^b_{{i-1}}})$ ($i=2,3,\ldots,n$) and the average return $\bar{r}^b = {\sum_{i=1}^n r_i^b}/{n}$. Then the  volatility in week $w$ is
{$$\sigma_b = \sqrt{  \frac{1}{n-1} \sum_{i=2}^n ( r_i^b-\bar{r}^b)^2  }\cdot 100.$$}
Notice that $n$ may vary from bond to bond and from week to week.
% RENAMED:
\item {\bf Number of trading days}: the number of days that bond $b$ is traded {during the week}.
\item {\bf Log(zero trade days)}: the log of the number of days that bond $b$  not traded {during the week}.
\item {\bf Proportion of buy/sell number}: estimated by counting the number of customer-buy orders and number of customer-sell orders in week $w$ and calculating the proportion of buys and sells for each bond $b$.
\item {\bf Proportion of buy/sell volume}: estimated by taking the total volumes (in dollars) for customer-buy orders and customer-sell orders in week $w$ and calculating  the proportion of buys and sells for each bond $b$.
\item  {\bf Trading activity}:  the log of the {\it number of trades} in the week.
\item {\bf Total volume}:  the weekly total trading volume {in dollars} of both customer-dealer trades and dealer-dealer trades.
\item {\bf Average price}: the weekly average trade price {in dollars}.
\item {\bf Coupon}: annual coupon payments paid by the issuer relative to the bond's face or par value. The coupon rate is the yield the bond paid on its issue date. This yield changes as the value of the bond changes, thus giving the bond's yield to maturity.
\item {\bf Duration}: an approximation of a bond's price sensitivity to changes in interest rates which is defined as
\begin{eqnarray*}
D^b = \sum_t \frac{\mbox{PV}(C^b_t)}{ \sum_t \mbox{PV}(C_t^b)} \times t,
\end{eqnarray*}
for bond $b$, where $C_t^b$ is the cash flow on date t, $PV(C^b_t)$ is its present value (evaluated at the bond's yield), and $\sum_t \mbox{PV}(C_t^b)$ is the total present value of the cash flows, which is equal to the bond's current price.
\item {\bf Years to maturity}:  the time to maturity date calculated in years.
  % RENAMED
\item {\bf Years since issuance}: the time since issued  date counted in years.
\item {\bf Amount outstanding}: the principal amount outstanding of a bond and is sometimes referred to as the notional amount.
\item {\bf Turnover}: { the volume of bonds {\color{red}traded} relative to the total volume of outstanding bonds.} The inverse of the turnover can be interpreted as the average holding time of the bond. For instance,   turnover of one implies an average holding time of about two weeks.
\item {\bf LIBOR-OIS rate}:  London inter-bank offer rate (LIBOR) as  the rate at which banks indicate they are willing to lend to other banks for a specified term of the loan; and  overnight indexed swap (OIS) rate as the rate on a derivative contract on the overnight rate. The term LIBOR-OIS spread is assumed to be a measure of the health of banks because it reflects the  default risk associated with lending to other banks.  In this analysis, the 1-month LIBOR-OIS rate is used to indicate the bank health condition over time.
\item {\bf Indicator of high yield (HY) or investment grade (IG) bond}: indicator of  the bond .

\item {\bf Indicator of different sectors}: including nine different sectors such as basic materials sector (S1), communications sector (S2), consumer \& cyclical sector (S3), consumer \& non-cyclical sector (S4), energy sector (S5), financial sector (S6), industrial sector (S7), technology sector (S8), and utilities sector (S9).

\end{itemize}
Table \ref{tab:features_stats} provides descriptive statistics of response variables and features.

\begin{table}[H]
  \centering\captionsetup{margin = -3.5cm}
  \setlength{\tabcolsep}{0pt}
  \begin{tabular}{lrrrrr}
    & \rule{2ex}{0pt}Mean & \rule{4ex}{0pt}std. & \rule{3ex}{0pt}q-25\% & \rule{2ex}{0pt}Median & \rule{2ex}{0pt}q-75\%\\\hline
    Bid-ask spread (bp) & 68.79 & 69.1 & 23.14 & 45.82 & 90.91 \\[0.2em]
    Volatility  &  0.785 & 0.582 & 0.388 & 0.646 & 1.039\\
    %12.41&9.21&6.13&10.21&16.43\\
    Trading activity& 1.28 & 0/35 & 1.04 & 1.26 & 1.51\\
    Log(\$ traded volume) & 6.90 & 0.63 & 6.50 & 6.94 & 7.33\\
    Nbe trading days & 4.41 & 0.80 & 4.00& 5.00& 5.00\\
    Log(zero trade days) & 0.12 & 0.18 & 0.00& 0.00 &0.30\\
    Prop. nbe buy & 0.45 & 0.18 & 0.33 & 0.45 & 0.57\\
    Prop. nbe sell & 0.55 & 0.18 & 0.43 & 0.55 & 0.67 \\
    Prop. \$ buy & 0.49 & 0.25 & 0.32 & 0.50 & 0.66\\
    Prop. \$ sell & 0.51 & 0.25 & 0.34 & 0.51 & 0.69\\
    Avg. price & 103.69 & 10.93 & 100.06 & 102.87 & 107.93\\
    Coupon & 4.69& 1.78 & 3.38 & 4.65 & 5.93\\
    Duration & 5.72 & 4.21& 2.75& 6.0& 8.0\\
    Years to maturity & 8.23 & 7.91& 3.0 & 6.0 & 8.0 \\
    Years since issuance & 3.99 & 2.93 & 2.0&3.0&5.0\\
    Turnover ($\times 10^{-2}$)& 1.80 & 6.10 & 0.30 & 0.80 & 1.90\\
    LIBOR-OIS & 0.21 & 0.09 & 0.14 & 0.20 & 0.25 \\
  \end{tabular}\\[.5em]
  \begin{tabular}{lrrclrr}
    & \rule{2ex}{0pt}Mean & \rule{4ex}{0pt}std. &\rule{4ex}{0pt}&& \rule{2ex}{0pt}Mean & \rule{4ex}{0pt}std. \\\cline{1-3}\cline{5-7}
    High yield & 0.27 & 0.44 & & Invest. grade & 0.73 & 0.44\\[0.2em]
    S: Basic Material & 0.03 & 0.18 && S: Communications & 0.15 & 0.38\\
    S: Consumer, Cyclical & 0.11 & 0.31 && S: Consumer, Non-cyclical & 0.14 & 0.35 \\
    S: Energy & 0.16 & 0.37 & & S: Financial & 0.27 & 0.44 \\
    S: Industrial & 0.07 & 0.25 && S: Technology & 0.07 & 0.25\\
    S: Utilities & 0.01 & 0.11 && & &\\
  \end{tabular}
  
  \caption{Statistics of the response variable and the features.}
  \label{tab:features_stats}
\end{table}

% ----


\paragraph{Hyperparameter selection.}
Specific to the regression models aforementioned, denote $\pmb{\mu}$ as the parameter for one of the regression models (for example, $\pmb{\mu} =(\lambda_e,\alpha)$ for EN).  Partition in log-scale is used for $m$ different hyperparameter values for $\pmb{\mu}$, and  the data is divided  into $K$ folds for  $K$-folds  cross-validation. For each {leave-out} fold $i$ ({the test set}),  the out of sample $R^2_i({\pmb{\mu}})$ is computed. Hence for each $\lambda$, there is  an empirical distribution of  $\tilde{R^2}({\pmb{\mu}}) = \{R^2_i({\pmb{\mu}}), i=1,2,\cdots,K\}.$ Denote ${\widehat{R^2}}(\pmb{\mu})$ and $\sigma_{R^2}(\pmb{\mu})$ as the mean and standard deviation of the empirical distribution with parameter $\pmb{\mu}$, and define the confidence interval by
\begin{eqnarray}\label{ci_1}
  {\frak{I}}_1(\pmb{\mu}) =\left[ {\widehat{R^2}}(\pmb{\mu}) - {\sigma_{R^2}(\pmb{\mu})\over\sqrt{K}}, %
  {\widehat{R^2}}(\pmb{\mu}) + {\sigma_{R^2}(\pmb{\mu})\over\sqrt{K}}\right].
\end{eqnarray}
Then  $\pmb{\mu}$ is picked such that the number of $ \tilde{R^2}(\pmb{\mu})$ in $ {\frak{I}}_1(\pmb{\mu})$ is maximized. Moreover, define
\begin{eqnarray}\label{ci_2}
{\frak{I}}_2(\pmb{\mu}) = \left[ {\widehat{R^2}}(\pmb{\mu}) - {\sigma_{R^2}(\pmb{\mu})}, %
  {\widehat{R^2}}(\pmb{\mu}) + {\sigma_{R^2}(\pmb{\mu})}\right].
\end{eqnarray}
Note that ${\frak{I}}_2(\pmb{\mu})$ in \eqref{ci_2} is a relaxation of ${\frak{I}}_1(\pmb{\mu})$ in \eqref{ci_1}. When the number of $ \{R^2_i({\pmb{\mu}})\}$ is not sensitive to $\pmb{\mu}$ in ${\frak{I}}_1(\pmb{\mu})$, one can compare ${\frak{I}}_2(\pmb{\mu})$ instead.


The training dataset consists of data from  Jan/01/2015 to Dec/31/2016, and the test dataset consists of data from  Jan/01/2017 to March/31/2017.  



\subsection{Results from OLS}
The estimation result is reported in Table \ref{OLS}. All but two of the estimated coefficients are statistically significant at any reasonable level of significance.%, which is not surprising because the sample size is large and we have strong prior information on related features. 
  The two exceptions are {{\it year to maturity} and {\it turnover}}.
  

  
\begin{itemize}
{
\item {The coefficients of {\it Prop number of buys} and {\it Prop number of sells} have the same sign but different values. The coefficient of {\it Prop number of buys} is roughly one third of the coefficient of {\it Prop number of sells}.
Similarly, both of the coefficients of {\it Prop buy volume} and {\it Prop sell volume} are positive. The coefficient of {\it Prop buy volume} is roughly half of the coefficient of {\it Prop sell volume}.}
This shows the asymmetric between customer buy orders and customer sell orders. This is consistent with  numerous studies \cite{FGP2016}  suggesting that dealers offer tighter quotes for larger trades than for smaller ones.  
\item The {\it Avg price} has a small effect on the bid-ask spread.
\item The indicators of different sectors have different coefficients but the overall values are small.
\item The {\it Log(Total volume)} coefficient is negative as expected. At round {-21}, the estimated coefficient implies that a 10000-bond increase in trade size in contracts, which would make a retail-size trade into a large institutional-size trade, and would reduce the bid-ask spread by {100 basis points}.
\item The {\it Indicator of investment grade bonds} coefficient is negative and the \emph{Indicator of high yield bonds} coefficient is positive. This is consistent with the well documented empirical findings: larger spreads for high yield bonds and smaller spreads for investment grade bonds.}
\end{itemize}



{\color{red}
\paragraph{Prediction power.}
 The distribution of the relative error is provided in Figure \ref{fig:relative_error}.
Errors  smaller than $0.3$ accounts for more than $70\%$ of  the testing dataset. The value of $R^2$ {\bf ??} indicates that this is a good out-of-sample performance.


\begin{figure}[H]
  \begin{center}
    \includegraphics[width=0.6\columnwidth]{figs/OOS_OLS.png}
    \caption{\label{fig:relative_error} Out-of-sample test on data during  Jan-March 2017.}
  \end{center}
\end{figure}
}



\subsection{Results from Two-Step Lasso}
%{\color{blue}[Renyuan \#1: (2) add comments on the difference between out-of-sample and cross-validation.]}

In this analysis,  20 different values of $\pmb{\mu}=\lambda_{l}$ are picked with partition in the range of $[10^{-1},10^{3}]$ in the log scale. 
The ranges of hyperparameters are different for two-step Lasso, Ridge and EN, shown in the figures of cross-validation scores,  Figures ~\ref{fig:cross_validation}, ~\ref{fig:cross_validation_l2}, and ~\ref{fig:cross_validation_EN}. 
The range is selected according to the sensitivity of  the model  with a larger prior partition grid.





{
Figure~\ref{fig:cross_validation} shows the 25\%, 50\% and 75\% percentiles of out-of-sample $\tilde{R}^2$ with different $\lambda_l$ values. One can see that all three 25\%, 50\% and 75\% curves decrease fast before {$\lambda_l^*=2.98$} and tend to be flat after $\lambda_l^*$. Also, both $\frak{I}_1(\lambda_l)$ and $\frak{I}_2(\lambda_l)$ are large when $\lambda_l=  \lambda_l^*$. Hence $\lambda_l^*$ is a good choice of the regularization level.
}
% The vertical line corresponds to $\lambda_l^*=0.29$.

 Table \ref{tab:R2_count_lasso} shows
 $\lambda_l$'s along with $\frak{I}_1(\lambda_l)$ and $\frak{I}_2(\lambda_l)$, in which the number of $\tilde{R}^2$ are the largest, respectively.
  
   
 Table \ref{LASSO_normal_scale} shows the features selected from the first step of the two-step
 the Lasso, with corresponding parameters {$\lambda^*_l = 1.13,$ $2.98$, and $7.85$}, respectively.
 It also shows the models from the OLS regression in the second step of
 the two-step Lasso. For instance,
 in Model L2 of Table \ref{LASSO_normal_scale} with $\lambda^*_l = 2.98$, the model is of the form with four features such that
{\begin{eqnarray}\label{eq:two_step_lasso_model}
\mbox{\it Bid-ask spread} =&&83.48\times \mbox{\it Volatility}+39.07 \times \mbox{{\it  Trading activity}}\\
&-&19.45\times  \mbox{\it Log(Total volume)} +0.23\times \mbox{\it Issued years}+86.
\end{eqnarray}}


{\color{red}
\paragraph{Prediction power.}
 The distribution of the relative error \eqref{eq:relative_error} is provided in Figure \ref{fig:relative_error2}.   Errors  smaller than $0.3$ account for more than $60\%$ of the testing dataset. The value of $R^2$ {\bf ??} suggests that  this is a good out-of-sample performance.
\begin{figure}[H]
  \begin{center}
    \includegraphics[width=0.6\columnwidth]{figs/OOS.png}
    \caption{\label{fig:relative_error2} Out-of-sample test of model \eqref{eq:two_step_lasso_model} on data during  01/01/2017-31/03/2017.}
  \end{center}
\end{figure}}


In addition, as seen  from Table~\ref{LASSO_normal_scale},

\begin{itemize}
\item The coefficient of {\it Volatility } is positive with value $83.48$. This is consistent with existing  theoretical and empirical studies in 
 market microstructure in  that a higher return volatility is predicted to lead a decreased liquidity (e.g., \cite{Stoll1978}).  
\item The coefficient of {\it Issued years} is positive with value {$0.23$}, which means a newly issued bond will have a small bid-ask spread. This is consistent with the work of \cite{KNP2016} which argued that recent and large issues are cheaper to trade than seasoned and small ones.
\item The number of trades per day $N$ and the trade volume $V$ (in dollars)  suggest the scale of ${N}/{\sqrt{V}}$ for the price  impact on the bid-ask spread in basis point.
Section \ref{regression_conclusion} provides  detailed analysis of this relationship.
\item Finally, $\lambda_l=7.85$ leads to the features of {\it Volatility} and  {\it Issued year} in model L3. Compared to model L2 with four features and $R^2=51.5\%$,  $R^2$ in EN3 drops to $43.22\%$. The model of four features, significantly  reduced from the original $26$ features, is preferable to EN3 in our view.  
\end{itemize}

It is worth noting that our findings are  supported by previous studies. For instance, \cite{CMMS2005} found that credit quality, the age of a bond, the size of a bond issue, the original
maturity value of a bond at issuance date, and provisions such as a call, put, or convertible options all have strong impact on liquidity. \cite{choi2019customer} showed that the trade size and the maturity date are important features to understand bid-ask spread. 





\subsection{Results from Ridge}


In this analysis, 20 different values of $\lambda_r$ are chosen for  partition in the log scale in the range of {$[10^2,10^{8}]$}.


Figure~\ref{fig:cross_validation_l2} shows the 25\%, 50\% and 75\% percentiles of out-of-sample $\tilde{R}^2$ with different $\lambda_r$ values. One can see that all three 25\%, 50\% and 75\% curves start to decrease at {$\lambda_r^*=1.27\cdot 10^{6}$}. Hence {$1.27\cdot 10^{6}$} is a good choice of the regularization level.


 Table \ref{tab:R2_count_ridge} shows
 $\lambda_r$'s along with $CI(\lambda_r)$ and $CI_2(\lambda_r)$, in which the number of $\tilde{R}^2$ are the largest, respectively. Table \ref{Ridge_normal_scale} shows the results of Ridge regressions with parameters  {$\lambda^*_r = 1.62\cdot 10^{4}, 6.95\cdot 10^{4}$ and $1.27\cdot 10^{6}$}.
  

The analysis by the Ridge regression is consistent with the findings from the two-step Lasso. In particular,
\begin{itemize}
\item When $\lambda_r$ goes up, the coefficients of the following features go to $0$ very fast: {\it Indicator functions of different sectors}, {\it Proportion of volume (or number) buys (or sells)}, {\it Turnover }, and {\it Number of trading days)}. Note that from Table \ref{Ridge_normal_scale} these features are also excluded from Model L3 and L4 of Table~\ref{LASSO_normal_scale}, which means that results from these two approaches are consistent.
\item  When $\lambda_r$ takes a large value {$6.95\cdot 10^{4}$}, the {\it Volatility}, the {\it Issued years}, the {\it Trading activity} and the {\it Log(Total volume)} are still significant. This is also consistent with the findings from Lasso in Table~\ref{LASSO_normal_scale}. 
\item Both two-step Lasso and Ridge regressions point to the significance of time value and special structure of bonds. The variable {\it years since issuance} is significant in two of the two-step Lasso models: L1 and L3, and all three Ridge regression models. 
\end{itemize}
The difference between Lasso and Ridge regression:
{\it Avg price} is not significant in all three two-step Lasso models whereas it is significant in all three Ridge models. This inconsistency is expected because of the collinearity among features.
When features are correlated, Lasso tends to select one feature from a group of correlated features, while Ridge  tends to penalize the group of correlated features towards the same coefficients \cite{citeulike:10520959}. Indeed, as shown in Model R1, R2 and R3, the coefficients of {\it Prop number of buys} and {\it Prop number of sells} have the same value but with different signs; the coefficients of {\it Prop buy volume} and {\it Prop sell volume} also have the same value but with different signs.
Additionally, the reappearance of {\it Avg price} in Model EN3 is due to this group effect too.


\subsection{Results from Two-Step EN}


Figure~\ref{fig:cross_validation_EN} shows the 25\%, 50\% and 75\% percentiles of out-of-sample $\tilde{R}^2$ with different $\lambda_e$ values given different $\alpha=0.2,0.5$ and $0.8$. 
When {$(\alpha,\lambda_e)=(0.5,10^{3})$ and $(\alpha,\lambda_e)=(0.8,10^{3})$}, more than 170 empirical $\tilde{R}^2$ falls into $\frak{I}_2$. This is because the hyperparameter over-penalizes the model  such that all the coefficients and the empirical $\tilde{R}^2$ are all nearly zero. Therefore these sets of hyperparameters should be excluded. 



Instead, for the analysis the following parameters are selected $(\alpha,\lambda_e)=(0.5,0.774)$, $(\alpha,\lambda_e)=(0.8,2.15)$, and $(\alpha,\lambda_e)=(0.5,129)$.
Parameter  $(\alpha,\lambda_e)=(0.8,2.15)$ leads to the following set of features: {\it Volatility}, {\it Number of trades}, {\it Log(Total volume)} and {\it Issued year}. This is consistent with the feature selection in two-step Lasso model L2.
$(\alpha,\lambda_e)=(0.5,129)$ leads to the features: {\it Volatility} and  {\it Average price} in model EN3. Compared with model EN2 with four features and $R^2=51.5\%$, the $R^2$ in EN3 drops to $42.62\%$. Similar to the argument for $L3$, model EN2 with four features is superior to  EN3, in our view.
 
Through all three different regression models, the consensus is that {\it Volatility} and {\it Issued years} are important features.



\subsection{Comparison between  TRACE Enhanced and  Standard TRACE dataset}
The comparison between TRACE Enhanced  and  TRACE Standard datasets for OLS and two-step LASSO is summarized here. 

Table \ref{OLS_trace_comparison} compares the OLS regression with data in  TRACE Enhanced  and  TRACE Standard from the same period 01/01/2015-12/31/2016. 
It shows similar $R^2$ values, with $55.4\%$ for TRACE Enhanced and $54.4\%$ for TRACE Standard. The relative difference between the regression coefficients is  small except for the following features.
\begin{itemize}
    \item {\it Prop Volume sell \$} and {\it Prop Volume buy \$}: For TRACE Enhanced, the coefficient of {\it Prop Volume buy \$} is 50\% larger than that of  {\it Prop Volume sell \$}. This relationship is reversed for TRACE Standard.  Further studies of the distribution of capped transactions show that 65\% of these transactions are customer sell orders. This contributes to  the changes of these two features in the TRACE Standard, as well as  the difference in regression coefficients. See  Figure \ref{fig:propo_buy_enhanced_standard}.
    \item {\it Turnover} and {\it Years to maturity}: The coefficients of these two features are much bigger for TRACE Standard. This difference is tolerable as neither of two features is significant $(p\ge0.1)$.
\end{itemize}

Comparing the two-step LASSO model on these two datasets, Table \ref{LASSO_standard_enhanced},   confirms similar conclusions: the outstanding features are consistent  and the regression coefficients are compatible.  







\begin{table}[H]
\centering
\small{
	%\renewcommand\thetable{5}
\caption{Two-step Lasso regression table: the impact  on bid-ask spread (in bp)\label{LASSO_standard_enhanced}}
\centering\setlength{\tabcolsep}{4pt}
\captionsetup{margin=-2.cm}
\begin{tabular}{@{}l
*{2}{S[table-format=4.4,table-number-alignment=center]}@{}}\toprule
                    &   {Enhanced TRACE} & {Standard TRACE}   \\ \midrule
Volatility            &      80.7218{***}                   & 72.96{***}\\
%Volatility        &      4.9159{***}      &      5.1053{***}         &       5.2836{***}             & 5.4709{***}\\
                       &        {(0.253)      }               &{(0.21)} \\
                  %       &    {  (0.020)    }      &        {(0.016)      }      &     { (0.014)    }           &{(0.015)} \\

 {Trading activity}            &         42.1450{***}        &    45.46{***}              \\
                     &            { (0.451)  }    &     { (0.496)  }     \\
 Log(Total Volume )              &        -21.1246{***}       &       -19.39{***}          \\
              &         {(0.252)  }         &      {   (0.261)  }           \\
      Years since issuance                               &       0.25{***}             &        0.32{***}       \\
           &             {(0.052)  }           &      {   (0.041) }       \\
Constant         &     86.1737          &     63.25      \\ \hline
N                                                                        &    152,408                      &130,716 \\
$R^2$                       &      52.8\%            &       52.5\%      \\ \bottomrule
%AIC                 &     17081.5   &      3251.0   &     15244.0   \\
\hline
\end{tabular}
\\ 
%\scriptsize{\textit{Dependent Variable:} Gender Bills (1 = bill proposal is related to women's issues; 0 otherwise).} \\
\scriptsize{Standard errors in parenthesis. Significance levels: * p$<$0.1, ** p$<$0.05, *** p$<$0.01. Two-tailed test.} \\
\scriptsize{Source: Enhanced TRACE (2015-2016).}
}
\end{table}



\begin{figure}[H]
  \begin{center}
    \includegraphics[width=0.6\columnwidth]{figs/buy_comparison_TRACE.png}
    \caption{\label{fig:propo_buy_enhanced_standard} Proportion of customer buy orders (in dollars).}
  \end{center}
\end{figure}
























\subsection{Conclusion: Main Features of  Bid-Ask Spread of Corporate Bonds}
\label{regression_conclusion}
%{\color{blue}[Renyuan \#2: add comments on out-of-sample-test and comparison between Standard TRACE and Enhanced TRACE.]}

We have performed different linear regressions for feature selection and for explaining the bid-ask spread using two kinds of variables: one describing the bond and the other characterizing the market context.
   Tables \ref{OLS} to \ref{Enet_normal_scale} summarize the results, with comparison to an OLS approach.  The recommendation based on these different penalization approaches is to  keep the ``version 2'' of the models: L2 for Lasso, R2 for Ridge and EN2 for EN regression.

Moreover, these regressions allow for computing an ``expected bid-ask spread'' for a given week, which can be used as a benchmark cost for TCA. In particular, 
  \begin{itemize}
  \item \emph{The volatility} is an important feature, as expected by empirical observations and the theory:
    the larger the volatility, the larger the bid-ask spread. It has been  observed in practice that an increase of 5\% of the volatility, that is $1/2$ of its standard deviation in our dataset, corresponds to an increase of the bid-ask spread by 25 basis points, which is around one third of its standard deviation.
  \item \emph{The number of trades per day} $N$ and \emph{the traded volume} $V$ (in dollars) are both important variables (in log units), with coefficient suggesting  ${\rm log}(N/\sqrt{V})$ being the faeture  impacting the bid-ask spread in the basis point.\footnote{
  The ridge regression suggests  the feature being in the form of  $\frac{N}{V}$, with an addition term of the average price. Possible explanation: penalization in the Ridge regression  tends to avoid large coefficients in the regression.}
    This implies that:
    \begin{itemize}
    \item for a given \emph{trading activity} $N$, the larger the traded volume, the smaller the bid-ask spread (in basis point);
    \item for a given traded volume in dollars, the lower the average trade size (i.e. the more trades), the large the bid-ask spread. 
    \end{itemize}
It is compatible with the documented stylized fact that for corporate bonds, small trade size obtain a worse bid-ask spread than large trades  \cite{FGP2016}.
  \item The value of the coupon and the duration of the corporate bond play a small role in the formation of the bid-ask spread (both with a positive coefficient).
  \item Last but not least, the \emph{Number of years to maturity} and the \emph{Years since issuance} are selected by our robust regressions. Keep in mind these two variables are linked, via the maturity of the bond, thanks to the relation:  {\it Year to maturity} = {\it Maturity} - {\it Years since issuance}. Hence naturally, the coefficient of \emph{year to maturity} is negative while the one of \emph{years since issuance} is positive: the further away from the maturity, the smaller the bid-ask spread (in basis point).
  
    This could support the market folklore that there is only a short period time after the issuance when coorperate bond trading is not too expensive  on secondary markets.
  \end{itemize}
  Other variables appeared in the OLS are not robust enough to be selected by penalized regressions. Removing these 17 variables from the regression only reduces the $R^2$ from around 0.55 to around 0.50, a minor price to pay for the increased robustness.  It is worth noticing that $R^2$ of all these OLS and regularized regressions are around 50\%, which is in line with the best results obtained in the academic literature: \cite{dn12bond} obtained $R^2$ between 0.50 and 0.80, while the $R^2$ of other studies were way below 0.50 (see Section \ref{sec:literature}).
  
  
Comparing the regression results between Standard TRACE and Enhanced TRACE (Table \ref{OLS_trace_comparison} for OLS and Table \ref{LASSO_standard_enhanced} for two-step LASSO) confirms  similar performance in terms of $R^2$ for these two datasets. One could choose either dataset for the bid-ask spread estimation, depending on the time-lag and the accuracy of the trade volume.


